Category-Level 6D Object Pose Estimation via Cascaded Relation and Recurrent Reconstruction Networks

Category-level 6D pose estimation, aiming to predict the location and orientation of unseen object instances, is fundamental to many scenarios such as robotic manipulation and augmented reality, yet still remains unsolved. Precisely recovering instance 3D model in the canonical space and accurately matching it with the observation is an essential point when estimating 6D pose for unseen objects. In this paper, we achieve accurate category-level 6D pose estimation via cascaded relation and recurrent reconstruction networks. Specifically, a novel cascaded relation network is dedicated for advanced representation learning to explore the complex and informative relations among instance RGB image, instance point cloud and category shape prior. Furthermore, we design a recurrent reconstruction network for iterative residual refinement to progressively improve the reconstruction and correspondence estimations from coarse to fine. Finally, the instance 6D pose is obtained leveraging the estimated dense correspondences between the instance point cloud and the reconstructed 3D model in the canonical space. We have conducted extensive experiments on two well-acknowledged benchmarks of category-level 6D pose estimation, with significant performance improvement over existing approaches. On the representatively strict evaluation metrics of $3D_{75}$ and $5^{\circ}2 cm$, our method exceeds the latest state-of-the-art SPD by $4.9\%$ and $17.7\%$ on the CAMERA25 dataset, and by $2.7\%$ and $8.5\%$ on the REAL275 dataset. Codes are available at https://wangjiaze.cn/projects/6DPoseEstimation.html.

==> figures/figure.tex <==
%previous tables
\iffalse


\begin{figure*}[t]
    \centering
    \begin{minipage}{1.0\textwidth}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/camera/val_00019_0006_0_pred-spd.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/camera/val_00024_0008_0_pred-spd.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/camera/val_00040_0001_0_pred-spd.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/camera/val_00062_0004_0_pred-spd.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/camera/val_00016_0001_0_pred-spd.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/camera/val_00015_0008_0_pred-spd.png}
    \end{minipage}
    \vfill
    \begin{minipage}{1.0\textwidth}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/camera/val_00019_0006_0_pred-ours.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/camera/val_00024_0008_0_pred-ours.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/camera/val_00040_0001_0_pred-ours.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/camera/val_00062_0004_0_pred-ours.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/camera/val_00016_0001_0_pred-ours.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/camera/val_00015_0008_0_pred-ours.png}
    \end{minipage}\vspace{5pt}
    \centering{(a) Comparative results with SPD~\cite{tian2020shape} on CAMERA25 dataset. Top row: results from SPD. Bottom row: Ours.}
    \vfill
    \vspace{5pt}
    \begin{minipage}{1.0\textwidth}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/real/test_scene_2_0324_0_pred-spd.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/real/test_scene_3_0465_0_pred-spd.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/real/test_scene_4_0095_0_pred-spd.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/real/test_scene_6_0487_0_pred-spd.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/real/test_scene_1_0172_0_pred-spd.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/real/test_scene_2_0187_0_pred-spd.png}
    \end{minipage}
    \vfill
    \begin{minipage}{1.0\textwidth}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/real/test_scene_2_0324_0_pred-ours.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/real/test_scene_3_0465_0_pred-ours.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/real/test_scene_4_0095_0_pred-ours.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/real/test_scene_6_0487_0_pred-ours.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/real/test_scene_1_0172_0_pred-ours.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative_red/real/test_scene_2_0187_0_pred-ours.png}
    \end{minipage}\vspace{5pt}
    \centering{(b) Comparative results with SPD~\cite{tian2020shape} on REAL275 dataset. Top row: results from SPD. Bottom row: Ours.}\vspace{3pt}
    \caption{Visual Comparison of 6D object pose and size recovered by ours and SPD~\cite{tian2020shape}.}
    \label{fig:qua_com}
\end{figure*}
\begin{figure*}[t]
    \centering
    \vfill
    \vspace{5pt}
    \begin{minipage}{1.0\textwidth}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/1_1.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/1_2.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/1_3.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/1_4.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/1_5.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/1_6.png}
    \end{minipage}
    \vfill
    \begin{minipage}{1.0\textwidth}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/2_1.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/2_2.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/2_3.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/2_4.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/2_5.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/2_6.png}
    \end{minipage}\vspace{5pt}
    \centering{(a) Comparative results with SPD~\cite{tian2020shape} on CAMERA25 dataset. Top row: results from SPD. Bottom row: Ours.}
    \vfill
    \vspace{5pt}
    \begin{minipage}{1.0\textwidth}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/3_1.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/3_2.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/3_3.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/3_4.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/3_5.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/3_6.png}
    \end{minipage}
    \vfill
    \begin{minipage}{1.0\textwidth}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/4_1.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/4_2.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/4_3.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/4_4.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/4_5.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/4_6.png}
    \end{minipage}\vspace{5pt}
    \centering{(b) Comparative results with SPD~\cite{tian2020shape} on REAL275 dataset. Top row: results from SPD. Bottom row: Ours.}\vspace{3pt}
    \caption{Visual Comparison of 6D object pose and size recovered by ours and SPD. The most obvious difference is marked with a red box. Apparently, our method produces more accurate 6D pose and size.}
    \label{fig:qua_com}
\end{figure*}


\begin{figure*}[!ht]
	\centering
	\includegraphics[width=\linewidth]{figures/vis.png}
	\caption{Visual Comparison of 6D object pose and size recovered by ours and SPD. The most obvious difference is marked with a red box. Apparently, our method produces more accurate 6D pose and size. \needcheck{To be changed}}
	\label{fig:qua_com}
\end{figure*} 


\begin{figure*}[t]
    \centering
    \begin{minipage}{1.0\textwidth}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/camera/val_00019_0006_0_pred_spd.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/camera/val_00024_0008_0_pred-spd.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/camera/val_00040_0001_0_pred-spd.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/camera/val_00062_0004_0_pred-spd.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/camera/val_00040_0001_0_pred-spd.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/camera/val_00062_0004_0_pred-spd.png}
    \end{minipage}
    \vfill
    \begin{minipage}{1.0\textwidth}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/camera/val_00019_0006_0_pred_ours.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/camera/val_00024_0008_0_pred-ours.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/camera/val_00040_0001_0_pred-ours.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/camera/val_00062_0004_0_pred-ours.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/camera/val_00040_0001_0_pred-ours.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/camera/val_00062_0004_0_pred-ours.png}
    \end{minipage}\vspace{5pt}
    \centering{(a) Comparative results with SPD~\cite{tian2020shape} on CAMERA25 dataset. Top row: results from SPD. Bottom row: Ours.}
    \vfill
    \vspace{5pt}
    \begin{minipage}{1.0\textwidth}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/real/test_scene_2_0324_0_pred-spd.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/real/test_scene_3_0465_0_pred-spd.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/real/test_scene_4_0095_0_pred-spd.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/real/test_scene_6_0487_0_pred-spd.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/real/test_scene_4_0095_0_pred-spd.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/real/test_scene_6_0487_0_pred-spd.png}
    \end{minipage}
    \vfill
    \begin{minipage}{1.0\textwidth}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/real/test_scene_2_0324_0_pred-ours.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/real/test_scene_3_0465_0_pred-ours.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/real/test_scene_4_0095_0_pred-ours.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/real/test_scene_6_0487_0_pred-ours.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/real/test_scene_4_0095_0_pred-ours.png}
        \includegraphics[width=0.163\linewidth]{figures/qualitative/real/test_scene_6_0487_0_pred-ours.png}
    \end{minipage}\vspace{5pt}
    \centering{(b) Comparative results with SPD~\cite{tian2020shape} on REAL275 dataset. Top row: results from SPD. Bottom row: Ours.}\vspace{3pt}
    \caption{Qualitative Comparison with SPD. \needcheck{To be changed}}
    \label{fig:qua_com}
\end{figure*}
\fi

%\subsection{temp}
% Please add the following required packages to your document preamble:


\iffalse
\begin{figure*}[t]
    \centering
    \begin{minipage}{1.0\textwidth}
        \includegraphics[width=0.245\linewidth]{figures/qualitative/camera/val_00019_0006_0_pred_spd.png}
        \includegraphics[width=0.245\linewidth]{figures/qualitative/camera/val_00024_0008_0_pred-spd.png}
        \includegraphics[width=0.245\linewidth]{figures/qualitative/camera/val_00040_0001_0_pred-spd.png}
        \includegraphics[width=0.245\linewidth]{figures/qualitative/camera/val_00062_0004_0_pred-spd.png}
    \end{minipage}
    \vfill
    \begin{minipage}{1.0\textwidth}
        \includegraphics[width=0.245\linewidth]{figures/qualitative/camera/val_00019_0006_0_pred_ours.png}
        \includegraphics[width=0.245\linewidth]{figures/qualitative/camera/val_00024_0008_0_pred-ours.png}
        \includegraphics[width=0.245\linewidth]{figures/qualitative/camera/val_00040_0001_0_pred-ours.png}
        \includegraphics[width=0.245\linewidth]{figures/qualitative/camera/val_00062_0004_0_pred-ours.png}
    \end{minipage}\vspace{5pt}
    \centering{(a) Comparative results with SPD~\cite{tian2020shape} on CAMERA25 dataset. Top row: results from SPD. Bottom row: Ours.}
    \vfill
    \vspace{5pt}
    \begin{minipage}{1.0\textwidth}
        \includegraphics[width=0.245\linewidth]{figures/qualitative/real/test_scene_2_0324_0_pred-spd.png}
        \includegraphics[width=0.245\linewidth]{figures/qualitative/real/test_scene_3_0465_0_pred-spd.png}
        \includegraphics[width=0.245\linewidth]{figures/qualitative/real/test_scene_4_0095_0_pred-spd.png}
        \includegraphics[width=0.245\linewidth]{figures/qualitative/real/test_scene_6_0487_0_pred-spd.png}
    \end{minipage}
    \vfill
    \begin{minipage}{1.0\textwidth}
        \includegraphics[width=0.245\linewidth]{figures/qualitative/real/test_scene_2_0324_0_pred-ours.png}
        \includegraphics[width=0.245\linewidth]{figures/qualitative/real/test_scene_3_0465_0_pred-ours.png}
        \includegraphics[width=0.245\linewidth]{figures/qualitative/real/test_scene_4_0095_0_pred-ours.png}
        \includegraphics[width=0.245\linewidth]{figures/qualitative/real/test_scene_6_0487_0_pred-ours.png}
    \end{minipage}\vspace{5pt}
    \centering{(b) Comparative results with SPD~\cite{tian2020shape} on REAL275 dataset. Top row: results from SPD. Bottom row: Ours.}\vspace{3pt}
    \caption{Qualitative Comparison with SPD. \needcheck{To be changed}}
    \label{fig:qua_com}
\end{figure*}


\begin{table*}[!ht]
\centering
\label{table:recurrent}
\caption{Evaluation of Recurrent Refinement Module.}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
\hline
\multirow{2}{*}{DATA} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Recurrent \\ Stages\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Loss \\ Weight\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Output \\ Stage\end{tabular}} & \multicolumn{6}{c}{mAP} \\ \cline{5-10} 
 &  &  &  & $3D_{50}$ & $3D_{75}$ & $5^{\circ}2cm$ & $5^{\circ}5cm$ & $10^{\circ}2cm$ & $10^{\circ}5cm$ \\ \hline
\multirow{6}{*}{CAMERA25} & 1 & 1:1:1 & 1 & 93.5 & 87 & 59.7 & 64.4 & 77.4 & 84.8 \\ \cline{2-10} 
 & \multirow{3}{*}{3} & \multirow{3}{*}{1:1:1} & 1 &93.7	& 87.8 &	62.2 &	66.8 &	78.4 &	85.7  \\
 &  &  & 2 & \textbf{93.7} & 88.6 & 62.9 & 67.9 & 78.6 & 85.8 \\
 &  &  & 3 & 93.6 & \textbf{88.7} & \textbf{62.6} & \textbf{67.2} & \textbf{78.8} & \textbf{85.6} \\ \cline{2-10} 
 & 3 & 4:2:1 & 3 & 93.3 & 87 & \textbf{64.4} & \textbf{68.5} & \textbf{78.9} & \textbf{85.6} \\ \cline{2-10} 
 & 3 & 1:2:4 & 3 & 93.5 & 88.3 & 62.3 & 66.8 & 78.3 & 85.5 \\ \hline
\multirow{6}{*}{REAL275} & 1 & 1:1:1 & 1 & 77.5 & 53.8 & 24.5 & 26.2 & 44.5 & 49.5 \\ \cline{2-10} 
 & \multirow{3}{*}{3} & \multirow{3}{*}{1:1:1} & 1 &  &  &  &  &  &  \\
 &  &  & 2 &  &  &  &  &  &  \\
 &  &  & 3 & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\ \cline{2-10} 
 & 3 & 4:2:1 & 3 &  &  &  &  &  &  \\ \cline{2-10} 
 & 3 & 1:2:4 & 3 &  &  &  &  &  &  \\ \hline
\end{tabular}
\end{table*}
\fi




\iffalse
\textbf{Category Performance Analysis.}
\begin{table*}[]
\centering
\caption{Category}
\label{table:category}
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
\multirow{2}{*}{DATA} & \multirow{2}{*}{Category} & \multicolumn{2}{c|}{NOCS} & \multicolumn{2}{c|}{SPD} & \multicolumn{2}{c}{IRNet} \\ \cline{3-8} 
 &  & $3D_{75}$ & $5^{\circ}2cm$ & $3D_{75}$ & $5^{\circ}2cm$ & $3D_{75}$ & $5^{\circ}2cm$ \\ \hline
\multirow{7}{*}{CAMERA25} & bottle &  &  &  &  &  &  \\ 
 & bowl &  &  &  &  &  &  \\ 
 & camera &  &  &  &  &  &  \\ 
 & can &  &  &  &  &  &  \\ 
 & laptop &  &  &  &  &  &  \\
 & mug &  &  &  &  &  &  \\ \cline{2-8} 
 & MEAN &  &  &  &  &  &  \\ \hline
\multirow{7}{*}{REAL275} & bottle &  &  &  &  &  &  \\ 
 & bowl &  &  &  &  &  &  \\ 
 & camera &  &  &  &  &  &  \\ 
 & can &  &  &  &  &  &  \\ 
 & laptop &  &  &  &  &  &  \\
 & mug &  &  &  &  &  &  \\ \cline{2-8} 
 & MEAN &  &  &  &  &  &  \\ \hline
\end{tabular}
\end{table*}
\fi

\iffalse
\begin{table*}[t]
%\begin{adjustbox}{width=0.7\textwidth,center}
\centering
\caption{Comparison of our method with other state-of-the-Art methods.}
\label{table:stoa}
%\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
\multirow{2}{*}{DATA} & \multirow{2}{*}{Method} & \multicolumn{6}{c}{mAP} \\ \cline{3-8} 
 & & $3D_{50}$ & $3D_{75}$ & $5^{\circ}2cm$ & $5^{\circ}5cm$ & $10^{\circ}2cm$ & $10^{\circ}5cm$ \\ \hline
\multirow{4}{*}{CAMERA25} & NOCS\cite{wang2019normalized} & 83.9 & 69.5 & 32.3 & 40.9 & 48.2 & 64.6 \\ %\cline{2-8} 
 & SPD\cite{tian2020shape} & 93.2 & 83.1 & 54.3 & 59 & 73.3 & 81.5 \\ %\cline{2-8} 
 %& CASS & - & - & - & - & - & - \\ %\cline{2-8} 
 & Ours & \textbf{93.8} & \textbf{88.0} & \textbf{72.0} & \textbf{76.4} & \textbf{81} & \textbf{87.7} \\ \hline
\multirow{4}{*}{REAL275} & NOCS\cite{wang2019normalized} & 78 & 30.1 & 7.2 & 10 & 13.8 & 25.2 \\ %\cline{2-8} 
 & SPD\cite{tian2020shape} & 77.3 & 53.2 & 19.3 & 21.4 & 43.2 & 54.1 \\ %\cline{2-8} 
 & CASS\cite{chencategory} & 77.7 & - & - & 23.5 & - & 58 \\ %\cline{2-8} 
 & Ours & \textbf{79.3} & \textbf{55.9} & \textbf{27.8} & \textbf{34.3} & \textbf{47.2} & \textbf{60.8} \\ \hline
\end{tabular}
%}
%\end{adjustbox}
\end{table*}

\begin{table}[ht]
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\hline
DATA & Method & Bottle & Bowl & Camera & Can & Laptop & Mug & Average \\ \hline
\multirow{2}{*}{CAMERA25} & SPD \cite{tian2020shape} & 1.81 & 1.63 & 4.02 & 0.97 & 1.98 & 1.42 & 1.97 \\
 & \textbf{Ours} &  \textbf{1.30} & \textbf{0.94} & \textbf{2.57}  & \textbf{0.81} & \textbf{0.87} & \textbf{1.04} & \textbf{1.18} \\ \hline
\multirow{2}{*}{REAL275} & SPD \cite{tian2020shape} & 3.44 & 1.21 & 8.89 & 1.56 & 2.91 & \textbf{1.02} & 3.17 \\
 & \textbf{Ours} & \textbf{2.99} & \textbf{0.95} & \textbf{7.57} & \textbf{1.31} & \textbf{1.25} & 1.19 & \textbf{2.53} \\ \hline
\end{tabular}
}
\end{table}

\begin{table}[t]
%\begin{adjustbox}{width=\textwidth}
\centering
\caption{Evaluation of Relation Reasoning Module}
\label{table:relation}
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
\multirow{2}{*}{DATA} & \multirow{2}{*}{Relation} & \multicolumn{6}{c}{mAP} \\ \cline{3-8} 
 & & $3D_{50}$ & $3D_{75}$ & $5^{\circ}2cm$ & $5^{\circ}5cm$ & $10^{\circ}2cm$ & $10^{\circ}5cm$ \\ \hline
\multirow{4}{*}{CAMERA25} & None & 93.5 & 87.0 & 59.7 & 64.4 & 77.4 & 84.8 \\ %\cline{2-8} 
 & MLP & 93.3 & 87.1 & 60.4 & 68.2 & 79.4 & 86.0 \\ %\cline{2-8} 
 & Non\_local & 93.2 & 87.0 & 65.6 & 70.2 & 80.4 & 86.7 \\ %\cline{2-8} 
 & Transformer & \textbf{93.4} & \textbf{87.1} & \textbf{70.9} & \textbf{75.7} & \textbf{80.5} & \textbf{87.3} \\ \hline
\multirow{4}{*}{REAL275} & None & 77.5 & 53.8 & 20.2 & 22.9 & 42.5 & 52.1 \\ %\cline{2-8} 
 & MLP & 77.1 & 51.1 & 23.9 & 29.6 & 46.2 & 59.3 \\ %\cline{2-8} 
 & Non\_local & 78.0 & 54.5 & 26.3 & 30.4 &  45.7 &  58.7 \\ %\cline{2-8} 
 & Transformer & \textbf{78.7} & \textbf{55.8} & \textbf{26.5} & \textbf{30.4} & \textbf{46.5} & \textbf{59.6}  \\ \hline
\end{tabular}
}
%\end{adjustbox}
\end{table}


\begin{table}[t]
\centering
\caption{Evaluation of Recurrent Reconstruction}
\label{table:recurrent}
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
\multirow{2}{*}{DATA} & \multirow{2}{*}{Step} & \multicolumn{6}{c}{mAP} \\ \cline{3-8} 
 &  & $3D_{50}$ & $3D_{75}$ & $5^{\circ}2cm$ & $5^{\circ}5cm$ & $10^{\circ}2cm$ & $10^{\circ}5cm$ \\ \hline
\multirow{4}{*}{CAMERA25} & Recurrent\_0 & 93.5 & 87.1 & 60.5 & 65.2 & 77.5 & 84.9 \\
 & Recurrent\_1 & \textbf{93.7} & 87.8 & 62.2 & 66.8 & 78.4 & 85.7 \\
 & Recurrent\_2 & 93.6 & 88.6 & \textbf{64.4} & \textbf{68.5} & \textbf{78.9} & \textbf{85.6} \\
 & Recurrent\_3 & 93.6 & \textbf{88.7} & 62.6 & 67.2 & 78.8 & \textbf{85.6} \\ \hline
\multirow{4}{*}{REAL275} & Recurrent\_0 & 77.5 & 55.4 & 19.9 & 23.9 & 45.6 & 57.7 \\
 & Recurrent\_1 & 77.5 & 55.6 & 22.2 & 24.7 & 46.3 & 60.1 \\
 & Recurrent\_2 & \textbf{81.9} & \textbf{57.0} & 24.2 & 25.7 & \textbf{46.4} & \textbf{60.2} \\
 & Recurrent\_3 & 80.5 & 56.5 & \textbf{24.5} & \textbf{26.2} & 44.5 & 59.5 \\ \hline
\end{tabular}
}
\end{table}

\fi

REAL275 contains 4300 real-world RGB-D image from 7 scenes for training, and 2750 real-world RGB-D images from 6 scenes for evaluation. 
